AccEar: Accelerometer Acoustic Eavesdropping with Unconstrained Vocabulary

With the increasing popularity of voice-based applications, acoustic eavesdropping has become a serious threat to users' privacy. While on smartphones the access to microphones needs an explicit user permission, acoustic eavesdropping attacks can rely on motion sensors (such as accelerometer and gyroscope), which access is unrestricted. However, previous instances of such attacks can only recognize a limited set of pre-trained words or phrases. In this paper, we present AccEar, an accelerometerbased acoustic eavesdropping attack that can reconstruct any audio played on the smartphone's loudspeaker with unconstrained vocabulary. We show that an attacker can employ a conditional Generative Adversarial Network (cGAN) to reconstruct highfidelity audio from low-frequency accelerometer signals. The presented cGAN model learns to recreate high-frequency components of the user's voice from low-frequency accelerometer signals through spectrogram enhancement. We assess the feasibility and effectiveness of AccEar attack in a thorough set of experiments using audio from 16 public personalities. As shown by the results in both objective and subjective evaluations, AccEar successfully reconstructs user speeches from accelerometer signals in different scenarios including varying sampling rate, audio volume, device model, etc.

==> NOTES-problemformulation.tex <==
\section{PROBLEM FORMULATION}
\label{sec:formulation}
In this paper, we focus on a side channel attack that exploits the accelerometer sensor to reconstruct spoken sentences played by the built-in smartphone speaker. 

A Inertial Measurement Unit (IMU), such as accelerometer and gyroscope, has high sensitivity to minute motions hence it readings are influenced by vibrations emitted by an active speaker which propagate to the IMU through the motherboard. Besides, the most popular operating systems of smartphone Android and iOS require no permission for an application to access IMU data. 
Therefore, an attacker can turn a IMU into a ``microphone'' to eavesdrop the sound played by the phone speaker without requesting access from the user. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%55
%in experimental setup
Our attack mainly targets Android devices since its prevalent share on smartphone market, i.e., $72.21\%$ reported by Statista\cite{statista}. 
It is worth noticing that the access of motion sensors does not require requesting permission before Android 12. To protect potentially sensitive information about users, an application on Android 12 needs permission to access IMU sensor when desired sampling rate is above $200Hz$~\cite{ratelimit}. In this work, we evaluate our attack scheme with multiple sampling rates to accommodate both the legacy and future permission policies of Android system.
Please note that our scheme could be easily implemented on iOS as well.
%app used for acquire acc data
Without loss of generality, in this paper, we apply a third-party application named \textit{Accelerometer Meter} running in the background to log the data of the three axes of the accelerometer and the corresponding timestamps when the audio is played by the speaker.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[h]
    \centering
    \includegraphics[scale=0.35]{figures/attack_model.pdf}
    \caption{Our attack scenario of accelerometer-based eavesdropping}
    \label{fig:attck_model}
\end{figure}
\subsection{Threat Model}
% We assume that the victim user has a high-end smartphone and the adversary is a spy app which can be installed in the victim user's phone disguised as any application. Whenever the victim user plays sound through the phone's built-in speaker, the spy app records acceleration data in the background in real time. It is important to note that since access to the accelerometer does not require requesting permission, we can obtain the data without the user's knowledge.

%threat model
We assume a spyware has been installed on the victim's smartphone that collects the accelerometer data in the background and try to reconstruct the voice from the collected data. 
When the built-in speaker of the victim's phone plays sound, the spyware records accelerometer data in the background in real-time.
In this work, we preform our attack by relying on data from the accelerometer since it has higher sensitivity than the gyroscope~\cite{ba2020learning}.
%In order to perform the eavesdropping stealthily without the user's awareness, it can setup a trigger for audio playing. This can be achieved by analyzing the high-frequency component of accelerometer data.
We assume the attacker has no prior information about the type of audio information emitting from the victim speaker, which implies the attacker is unable to classify a handful of audio signals (i.e., words or numbers). 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%to add into MOTIVATION in INTRODUCTION
\subsection{Attack Scenarios}
% This paper aims to reconstruct the audio played by the phone through acceleration data. It is important to note  that our model is not limited to the hot words, but can eavesdrop unconstrained vocabulary played by the phone speaker, which greatly increases the amount of information we can obtain. Based on this, we can use the proposed system to attack smartphone users and their contacts.
This paper aims to reconstruct the audio played by the phone through acceleration data. 
It is important to note  that our model is not limited to the hot words, but can eavesdrop unconstrained vocabulary played by the phone speaker, which greatly increases the risk of information leakage. Hence the attacker can adopt \pname to attack smartphone users and their contacts.

For a smartphone user, the attacker can pilfer his/her voice memo, which may contain confidential or privacy information such as account passwords, schedules, etc. When a user uses voice navigation, we can steal the user's location information through the sounds of navigation broadcast; when a user plays an audio containing the specific product name, we can infer the user's preferences from the reconstructed information, which is greatly valuable to personalized recommendations; when a user uses voice verification code, we can steal the verification code to attack the user.

For contacts, when a contact talks, videos, or sends voice messages with a user via smartphone, we can reconstruct the contact's voice to steal important information.
% \par Note that the information we steal is often of greater value when the target of the attack is a celebrity, so this paper mainly performs experiments for celebrities.

==> System_overview.tex <==
\begin{figure*}[h]
    \centering
    \includegraphics[scale=0.7]{figures/system.pdf}
    \caption{Architecture of AccEar system}
    \label{fig:system}
\end{figure*}
\section{SYSTEM OVERVIEW}
\label{sec:overview}
In this paper, the accelerometer is used to eavesdrop on the smartphone, and the whole process is shown in Fig.~\ref{fig:system}, which can be divided into three parts: data collection, pre-processing, and speech reconstruction.
\subsubsection*{\textbf{Data Collection}} When the smartphone's speaker plays audio, the spy app running in the background starts to record and store the data of the three axes of the accelerometer and the corresponding timestamps.
\subsubsection*{\textbf{Preprocessing}} We linearly interpolate the collected raw acceleration data to fix the time interval between the data. Then the interpolated data is subjected to a STFT to obtain the spectral characteristics of the data, and a spectrogram is drawn as input for the speech reconstruction.
\subsubsection*{\textbf{Speech Reconstruction}} We input the spectrogram of the acceleration data generated in the preprocessing stage into a pre-trained cGAN (conditional generative adversarial network), which adjusts the spectrogram of the acceleration data at the pixel level to obtain the Mel spectrogram of the audio we want to reconstruct.  Then, we use the Griffin-Lim algorithm to convert the generated Mel spectrogram into audio.


==> implementation.tex <==
\section{Implementation}
\subsection{Experimental setup and Datasets}
Introduce our experiment equipment and datasets.
\subsection{Evaluation indicator}
Introduce our evaluation indicator.
\subsection{Performance}
%\subsubsection{Different scenarios}
% a. Different scenarios
% \par List out different scenarios (such as mobile phones on the table or handheld mobile phones) of experimental data, verify the validity of the model.
% %\subsubsection{Different volume}
% \par b. Different volume
% \par List the experimental data under different volume.
% %\subsubsection{Different mobile phone}
% \par c. Different mobile phone
% \par List the experimental data under different mobile phone.
% \par 1.	在100$\%$音量，安静房间，手机静置在桌子上，手机型号为华为mate40 pro的条件下，分别训练出各位名人的模型。
% \par 2.	采集不同音量（20$\%$，40$\%$，60$\%$，80$\%$，100$\%$）下，安静房间，手机放在桌子上，手机型号为华为mate40 pro的数据，在1中训练的模型上进行测试。
% \par 3.	采集不同姿势（手持手机和将手机放在桌子上）下，100$\%$音量，安静房间，手机型号为华为mate40 pro的数据，在1中训练的模型上进行测试。
% \par 4.	采集不同手机型号（oppo reno6 pro，三星S21+，华为mate40 pro）下，安静房间，手机放在桌子上的数据，在1中训练的模型上进行训练。
% \par 5.	采集不同噪声背景（安静房间，咖啡厅，酒吧，火车站等）下，100$\%$音量，手机放在桌子上的数据，在1中训练的模型上进行测试。
% 这个具体的步骤是一共三部手机，在上述场景中，将手机1，2放在一起，手机3放置在安静地方的桌子上，然后将手机1与手机3接通，手机2最大音量播放测试集中的数据，手机3录音通话并记录加速度计的数据。
% \par 6. 采集不同采样频率（200hz, 250hz,300hz等比较低的频率)下，在100$\%$音量，安静房间，手机静置在桌子上的数据，这个如果效果不理想就不写进论文。
% \par 7.	利用名人1的模型测试名人2，3，4号的数据，以测试模型的通用性。
% \par 8.	利用多个人的数据一起训练的模型测试另外人的数据，以测试模型的通用性。
% \par 9.	利用中文、英文混合起来的数据集训练模型，用来测试中文名人和英文名人的数据。

